A Game-Theoretic Approach to the Study of Blockchain's Robustness

Blockchains have sparked global interest in recent years, gaining importance as they increasingly influence technology and finance. This thesis investigates the robustness of blockchain protocols, specifically focusing on Ethereum Proof-of-Stake. We define robustness in terms of two critical properties: Safety, which ensures that the blockchain will not have permanent conflicting blocks, and Liveness, which guarantees the continuous addition of new reliable blocks. Our research addresses the gap between traditional distributed systems approaches, which classify agents as either honest or Byzantine (i.e., malicious or faulty), and game-theoretic models that consider rational agents driven by incentives. We explore how incentives impact the robustness with both approaches. The thesis comprises three distinct analyses. First, we formalize the Ethereum PoS protocol, defining its properties and examining potential vulnerabilities through a distributed systems perspective. We identify that certain attacks can undermine the system's robustness. Second, we analyze the inactivity leak mechanism, a critical feature of Ethereum PoS, highlighting its role in maintaining system liveness during network disruptions but at the cost of safety. Finally, we employ game-theoretic models to study the strategies of rational validators within Ethereum PoS, identifying conditions under which these agents might deviate from the prescribed protocol to maximize their rewards. Our findings contribute to a deeper understanding of the importance of incentive mechanisms for blockchain robustness and provide insights into designing more resilient blockchain protocols.

==> Appendices/Pseudo-Randomness.tex <==
\chapter{Pseudo-Randomness in Ethereum}\label{chap:Pseudo-Randomness}

==> Chapters/RelatedWork.tex <==
% \chapter{Related Work on Blockchain Analysis} \label{chap:RelatedWork}

% \minitoc

% \chapterLettrine{O}{ur} work during this thesis revolves around the case study of Ethereum Proof-of-Stake. 
% \Yackolley{Il ne faudrait pas préciser de quelle version on parle ? Ou rappeler ici quand le protocol a été introduit} 
% We contribute to the field by formalizing the protocol, defining properties, presenting attacks against these properties, and then analyzing the strategies of rational validators. In this chapter, we present the related work corresponding to each of these efforts.


% \

% \section{Blockchain Formalization}

% The category of papers that aim to formalize to describe blockchains includes all the \emph{white papers}. These are articles explaining the main features of a protocol, often written by the team behind the blockchain. This trend started in 2008 with the first blockchain, Bitcoin \cite{nakamoto_peer_2008}, and has been followed almost religiously by subsequent protocols. Ethereum is no exception, having released its first white paper in 2014 \cite{buterin_next_2014} when the Ethereum blockchain operated with a PoW consensus.

% Following the release of a white paper by a protocol's team, other papers have emerged to challenge or complement the blockchain's description. For Bitcoin, this is exemplified by the work of Garay et al. \cite{garay_bitcoin_2015}, who analyzed the protocol's pseudo-code and deduced some of its properties. Similarly, Amoussou-Guenou et al. \cite{amoussou_dissecting_2019} proved the correctness of the Tendermint protocol, thereby complementing the initial white paper \cite{buchman_latest_2018}.  Alturki et al. \cite{alturki_towards_2019} used a proof assistant to prove the safety of the Algorand’s blockchain \cite{chen_algorand_2019}. Similarly, García-Pérez and Schett \cite{garcia_deconstructing_2019}provided a formal correctness proof of the Stellar Consensus Protocol (SCP). Amores-Sesar et al. \cite{amores_security_2020} study revealed that the  Ripple protocol might violate both safety and liveness, challenging the initial claims of Ripple's Byzantine fault tolerance.

% The first section of our work have a similar aim. We extract the pseudo-code from the Ethereum specifications \Sara{from specifications? white paper? pseudo-code?} to formalize its properties. The most recent Ethereum white paper was released to explain the new protocol following the transition from PoW to PoS \cite{buterin_combining_2020}.

% Outside of this line of work focusing on specific protocols, other efforts have aimed to provide formal foundations for blockchains. Anceaume et al. \cite{anceaume_abstract_2018} proposed a formalization of blockchains and their evolutions as Block Trees. The work of Anceaume et al. \cite{anceaume_finality_2021} described the different ways blockchains can ensures that block permanently belong to the chain, finalizing them. 
% We rely on the definitions of Block Tree and finality to express the properties of the Ethereum protocol. 

% \section{Attacks and Vulnerabilities}
% \TODO{Mettre le tableau des attacks pour cette section} A considerable amount of work has been focused on identifying protocol vulnerabilities. The most famous example is probably the seminal work of Eyal and Sirer \cite{eyal_majority_2018}, which presents the selfish mining attack on Bitcoin. They show that in Bitcoin (and proof-of-work in general), miners can benefit from deviating from the prescribed protocol by withholding blocks for a while, to the detriment of honest miners. Many other examples exist: for instance, Amoussou-Guenou et al. \cite{amoussou_correctness_2018} pointed out a liveness vulnerability in the Tendermint protocol, and Neuder et al. \cite{neuder_defending_2020} presented an attack where nodes can reorganize Tezos' Emmy+ chain and then perform a double-spend attack. The protocol has been updated since then for a more robust solution proposed by Astefanoaei et al. \cite{astefanoaei_ternderbake_2021}.

% Our work focuses on Ethereum, which is no stranger to protocol attacks. Neu et al. \cite{neu_ebb_2021} exhibited a balancing attack, highlighting the shortcomings of a consensus mechanism divided into two layers (finality gadget and fork choice rule). Mitigation against this attack was proposed, but Neu et al. \cite{neu_two_2022} overcame this mitigation with a new balancing attack. Schwarz-Schilling et al. \cite{schwarz_three_2021} presented reorg attacks  \Sara{what is a reorg attack?}
% , revealing that proposers could gain by disturbing the protocol by releasing their blocks late. 

% We contribute to this line of work by identifying flaws on the Ethereum PoS protocol. First, we outline a flaw regarding the liveness of the current Ethereum Proof-of-Stake protocol, emphasizing the importance of reconciling availability and finality. Our approach differs from Galletta et al. \cite{galletta_resilience_2023}, who aim to formally verify the \textit{Hybrid Casper} protocol \cite{buterin_casper_2017}, focusing on an outdated version. We formalize the current implemented version of the protocol through pseudo-code and expose a liveness attack on the protocol.

% Nakamura \cite{nakamura_prevention_2019} presented an attack called \textit{splitting attack}, in which the adversary sends messages to split the set of validators. However, Nakamura assumes that the adversary needs to control and manipulate network delays, which is a strong and potentially unrealistic assumption. More recently, Schwarz-Schilling et al. \cite{schwarz_three_2021} demonstrated through experiments that attackers can predict the proportion of validators receiving a given message within a specific timeframe with sufficient accuracy. This contradicts Nakamura's claim that the attack necessitates the adversary to control network delay. Our work presents a form of the splitting attack based on the weaker assumption that the adversary knows the network delay (in line with Schwarz-Schilling et al. \cite{schwarz_three_2021}) but does not control it. 
% \Yackolley{J'aurais mis ce dernier paragraphe avant, et avoir un paragraphe entier sur tes contribution. Je pense aussi que comme tu donnes une intuition du problème du type d'adversaire, tu peux aussi donner une intuition de ce qu'est une balancing attack (voir splitting aussi). Comme ça tu pourrais ddétailler en quoi la division en 2 protocols interconnectés est problématique et que ce n'est pas le cas des blockchains style BFT classiques}

% \subsection{Incentives}

% Very few efforts in the literature have taken the incentive mechanism of protocols into account to evaluate how Byzantine validators could exploit it.
% Initial efforts were made to intertwine the study of incentives with considerations of liveness and safety properties of the Ethereum protocol \cite{buterin_incentives_2020}. However, this early exploration discussed a preliminary version of the protocol \cite{buterin_casper_2017} and did not include an analysis of the inactivity leak. The inactivity leak is the mechanism that penalize inactive validators by reducing their stake. The most recent version of the protocol by its founder \cite{buterin_combining_2020} does not mention this mechanism. The inactivity leak still lacks a detailed examination, and our work aims to fill this gap.

% While mechanisms similar to Ethereum's inactivity leak exist elsewhere (e.g., \cite{wood_polkadot_2016, goodman_tezos_2014}), to the best of our knowledge, there has not been an analysis of the risk associated with potentially draining honest stake in a Byzantine-prone environment. \Yackolley{peut être préciser aussi sur la correction/les propriétés du protocole de consensus particulièrement, surtout que le paragraphe juste après semble être une contradiction. Et comme dans le cas précédent, ce serait bien de mettre tes contribution à la toute fine je trouve}

% An investigation linking penalties with the actions of Byzantine validators is presented by Zhang et al. \cite{zhang_attestation_2023}. This work demonstrates how Byzantine validators can maliciously cause attestation penalties for honest validators. Although similar in scope, we focus on more substantial penalties, i.e., the inactivity penalties and slashing. During the inactivity period, attestation penalties tend to be less significant.

% \section{Rational Agents in Blockchain}
% Incentives are not often considered in the distributed systems field; however, game theory addresses this gap.

% Following the influential work of Eyal and Sirer \cite{eyal_majority_2014, eyal_majority_2018}, subsequent works (e.g., \cite{grunspan_selfish_2020, nayak_stubborn_2016, sapirshtein_optimal_2016, bar_efficient_2020}) use game-theoretic tools to analyze the maximum gain a rational miner can achieve by selfish mining, i.e., deviating from the proof-of-work protocols by withholding found blocks to gain an advantage in mining subsequent blocks. 
% Also considering only rational participants, the work of Biais et al. \cite{biais_blockchain_2019} proves that while playing the proof-of-work game and following the longest chain’s rule is an equilibrium -where no participant can improve their outcome by changing their strategy-, multiple other equilibria exist where forks may persist. 

% These works do not apply to Ethereum since its PoS mechanism does not confer an advantage to block proposers who gain knowledge of a block sooner. The chain continues at a fixed pace, and block proposers are selected pseudo-randomly.

% Comparing our work to the game theory literature on the Ethereum PoS \emph{consensus}, Roughgarden \cite{roughgarden_transaction_2020} conducted a game-theoretic analysis of an Ethereum Improvement Proposal (EIP) to evaluate its impact on transaction and proposer rewards considering rational agents. Many works focus on MEV (Maximal Extractable Value), which involves taking advantage of the transaction ordering in a block. 
% In contrast, we focus on game-theoretic analyses affecting the consensus directly. We differ from works like \cite{bhudia_game_2023}, which consider the possibility of making ransom demands without being detected. Schwarz-Schilling \cite{schwarz_three_2022} studies the optimal timing for proposers to propose their blocks, while we analyze which block the proposer should build upon.

% Our endeavor is closest to the work of Carlsten et al. \cite{carlsten_instability_2016} and Tsabary and Eyal \cite{tsabary_eyal_2018}. They study selfish behavior in Bitcoin using game theory when the \emph{only} source of rewards is transaction fees (no more coinbase transactions). They show that the Bitcoin blockchain becomes unstable since block miners fork the Bitcoin blockchain to obtain the most lucrative transactions. 
% Ethereum PoS does not reward block proposers with coinbase transactions; however, the presence of attesters and a different fork choice rule than Bitcoin's makes the analysis more complex. We focus on analyzing the behavior of block proposers and attesters in Ethereum PoS using game theory and demonstrate that the protocol is stable, even though one proposer can gain more than following the prescribed strategy due to the initial asynchronous setting. Moreover, transaction fees do not play a crucial role in our analysis due to rewards stemming from attestations.

% At the intersection of distributed systems, which model agents as either honest or Byzantine, and game theory, which models agents as rational, a mixed model was proposed: BAR (Byzantine, Altruistic, and Rational) \cite{abraham_distributed_2011}. However, the complexity of the analysis rises quickly with so many types of agents. The work of Halpern and Vilaça \cite{halpern_rational_2016} considers rational participants who can fail by crashing. They prove that in such a setting, there is no ex-post Nash equilibrium solving the fair consensus problem. Amoussou et al. \cite{amoussou_rational_2020} consider agents being either rational or Byzantine, exhibiting different equilibrium depending on the proportion of each. \Yackolley{je ne suis pas trop fan de la structure des références dans la section rationnelle. Ça à l'air un peu fouilli et c'est un peu compliqué à suivre. Est-ce que tu considères les Byzantins? ça passe de Po* à BFT à Po*. Je pense qu'il faut restructurer un peu. On pourra en parler en une petite réunion rapidement. N'oublie pas le papier (On incentive compatible role-based reward distribution in algorand)} \Sara{je suis d'accord avec Yackolley. Il y a aussi pour la PoS nakamoto style le "nothing at stake pb et les travaux de Saleh à citer}.


